ProReco: A Process Discovery Recommender System

Process discovery aims to automatically derive process models from historical execution data (event logs). While various process discovery algorithms have been proposed in the last 25 years, there is no consensus on a dominating discovery algorithm. Selecting the most suitable discovery algorithm remains a challenge due to competing quality measures and diverse user requirements. Manually selecting the most suitable process discovery algorithm from a range of options for a given event log is a time-consuming and error-prone task. This paper introduces ProReco, a Process discovery Recommender system designed to recommend the most appropriate algorithm based on user preferences and event log characteristics. ProReco incorporates state-of-the-art discovery algorithms, extends the feature pools from previous work, and utilizes eXplainable AI (XAI) techniques to provide explanations for its recommendations.

==> log_table.tex <==
\begin{table}[H]
\centering
\caption{Statistics describing our data set of event logs.}
\label{logs}
\begin{tabularx}{\textwidth}{|l|X|X|X|X|X|X|}
\hline
\textbf{Name} & \textbf{No. of Logs} & \textbf{No. of Cases} & \textbf{No. of Events} & \textbf{No. of Activities} & \textbf{Trace Length Range} & \textbf{No. of Variants} \\ \hline
PDC 2020 & 192 & 1k & 6.7k--66k & 14--36 & 3--300 & 503--1k \\ \hline
Streams & 750 & 100--1k & 900--13.5k & 15--16 & 2--83 & 22--204 \\ \hline
Encoding & 140 & 1k & 10k--44k & 22--406 & 1--50 & 383--1k \\ \hline
BPIC12 & 4 & 5k--13k & 31k--262k & 7--24 & 2--175 & 17--4.3k \\ \hline
BPIC13 & 2 & 1k--7k & 6k--65k & 4 & 1--123 & 183--1.5k \\ \hline
Env. permit & 1 & 1.4k & 8.5k & 27 & 1--25 & 116 \\ \hline
Helpdesk & 1 & 4.5k & 21k & 14 & 2--15 & 226 \\ \hline
Sepsis & 1 & 1k & 15k & 16 & 3--185 & 841 \\ \hline
CC-2019 & 1 & 20 & 1394 & 29 & 52--118 & 20 \\ \hline
Daily Activities & 8 & 6--43 & 368--4.2k & 14--19 & 20--134 & 6--43 \\ \hline
Hospital Billing & 1 & 100k & 451.3k & 18 & 1--217 & 1020 \\ \hline
Road Traffic M. &1 &  150.3k & 561.5k & 11 & 2--20 & 231 \\ \hline
Artificial & 785 & 1k--1.5k & 1k--88.2k  & 1--199 &  1--198 & 1--1.5k \\ \hline
In total: & 1887 & 20--150.3k & 900--561.5k & 1--406 & 1--300 & 1--1.5k \\ \hline
\end{tabularx}
\end{table}

==> sections/related.tex <==
\section{Related Work}\label{sec:related}
